A Database System for State Management in Stateful Network Service Function Chains [Vision]

Network Function Virtualization (NFV) heralds a transformative era in network function deployment, enabling the orchestration of Service Function Chains (SFCs) for delivering complex and dynamic network services. Yet, the development and sustenance of stateful SFCs remain challenging, with intricate demands for usability in SFC development, performance, and execution correctness. In this paper, we present DB4NFV, a database system designed to address these challenges. Central to DB4NFV is the integration of transactional semantics into the entire lifecycle of stateful SFC, a core idea that enhances all aspects of the system. This integration provides an intuitive and well-structured API, which greatly simplifies the development of stateful SFCs. Concurrently, transactional semantics facilitate the optimization of runtime performance by efficiently leveraging modern multicore architectures. Moreover, by encapsulating state operations as transactions, DB4NFV achieves robustness, even at the entire chain level, ensuring reliable operation across varying network conditions. Consequently, DB4NFV marks a substantial forward leap in NFV state management, leveraging transactional semantics to achieve a harmonious blend of usability, efficiency, and robustness, thus facilitating the effective deployment of stateful SFCs in contemporary network infrastructures.

==> Sections/6_Related_Works.tex <==
\section{Related Work}
\label{sec:related}
The field of Network Function Virtualization (NFV) has witnessed considerable progress. Yet, current NFV frameworks~\cite{sherry2015rollback, rajagopalan2013pico, gember2014opennf, khalid2019correctness, woo2018elastic, rajagopalan2013split} struggle to efficiently manage VNF states while maintaining \textit{chain output equivalence} (COE).

Existing NFV frameworks primarily focus on ensuring state access availability. For instance, FTMB~\cite{sherry2015rollback} and Pico Replication~\cite{rajagopalan2013pico} discard state changes during failure recovery, while Split/Merge~\cite{rajagopalan2013split} ensures state availability during traffic reallocation. However, these frameworks operate under the assumption that no states are shared across VNF instances.

Managing shared mutable VNF states and satisfying COE requirements is a daunting task. OpenNF~\cite{gember2014opennf} and S6~\cite{woo2018elastic} guarantee consistency for shared states within the same VNF, but they fail to support chain-wide consistency requirements, including the chain-wide ordering needed by the trojan detector, as well as ensure state consistency during duplicated instance suppression and chain-wide failure recovery.

Among these, the CHC framework~\cite{khalid2019correctness} stands out for its attempt to fully accommodate COE requirements. Yet, it also has limitations. Its coarse-grained approach to managing cross-flow state results in considerable overhead. CHC's strategy for caching or flushing state objects, based on upstream traffic partitioner information, leads to frequent transfers between cache and main memory, resulting in high communication overhead. Moreover, the employment of mechanisms like locks to preserve consistency across multiple instances incurs additional overhead.
% Recognizing the necessity of ,  address this issue. 
% \subsection{Limitations of Related Works}
% \label{subsec:limitations}
% While the field of NFV has seen extensive research, leading to the proposal of several VNF frameworks~\cite{sherry2015rollback, rajagopalan2013pico, gember2014opennf, khalid2019correctness, woo2018elastic, rajagopalan2013split}, current solutions struggle to simultaneously assure efficient VNF state management and maintain \textit{chain output equivalence} (COE).

% Frameworks such as FTMB~\cite{sherry2015rollback}, Pico Replication~\cite{rajagopalan2013pico}, and Split/Merge~\cite{rajagopalan2013split} have mainly prioritized state access availability. These approaches focus on ensuring state availability during traffic reallocation and recovering from failures by discarding state changes, which limits their practicability to real-world scenarios.

% Recognizing the necessity of managing shared states within a single VNF, frameworks like OpenNF~\cite{gember2014opennf} and S6~\cite{woo2018elastic} have taken steps in this direction. Despite this recognition, they still struggle to meet the stringent requirements of COE, such as maintaining state consistency during instances' replication and ensuring state access ordering.

% The challenge of managing shared VNF states while satisfying COE requirements is significant. Several existing frameworks~\cite{bremler2016openbox, meng2019micronf, palkar2015e2, rajagopalan2013split, gember2014opennf, khalid2019correctness, woo2018elastic} evade these challenges by either neglecting cross-flow states or assuming perfect traffic partitioning. These approaches effectively avoid the complications of state sharing among instances. 

% While some frameworks, such as OpenNF~\cite{gember2014opennf}, CHC~\cite{khalid2019correctness}, and others~\cite{woo2018elastic, rajagopalan2013split}, attempt to maintain cross-flow state consistency during execution, their solutions prove inadequate under dynamic network conditions, including instance failure or traffic reallocation.

% The CHC framework~\cite{khalid2019correctness}, while noteworthy for attempting to fully support COE requirements, has its own limitations. Its method for managing cross-flow state is coarse-grained, resulting in considerable overhead. Specifically, CHC's decision-making process on caching or flushing state objects, based on upstream traffic partitioner information, leads to frequent state object transfers between cache and main memory. This causes high communication overhead. Additionally, the use of mechanisms like locks to maintain consistency across multiple instances introduces further overhead.


% Revised:

% "\subsection{Limitations of Related Works}
% \label{subsec:limitations}

% Network Function Virtualization (NFV) is a research-intensive field that has produced a multitude of Virtual Network Function (VNF) frameworks~\cite{sherry2015rollback, rajagopalan2013pico, gember2014opennf, khalid2019correctness, woo2018elastic, rajagopalan2013split}. However, existing solutions continue to wrestle with the task of achieving efficient VNF state management while also maintaining \textit{chain output equivalence} (COE).

% Several frameworks, such as FTMB~\cite{sherry2015rollback}, Pico Replication~\cite{rajagopalan2013pico}, and Split/Merge~\cite{rajagopalan2013split}, chiefly prioritize state access availability. Their primary focus is to ensure state availability during traffic reallocation and recovery from failures, often by disregarding state changes. The key limitation of these frameworks arises from the assumption that there are no shared states across VNF instances, which limits their practical applicability.

% Frameworks like OpenNF~\cite{gember2014opennf} and S6~\cite{woo2018elastic} make advancements in this area by managing shared states within a single VNF. Yet, they struggle to fulfill the stringent requirements of COE, particularly in maintaining state consistency during instances' replication and ensuring proper state access ordering.

% It is a significant challenge to manage shared VNF states while satisfying COE requirements. Many existing frameworks~\cite{bremler2016openbox, meng2019micronf, palkar2015e2, rajagopalan2013split, gember2014opennf, khalid2019correctness, woo2018elastic} circumvent these difficulties by either neglecting cross-flow states or assuming perfect traffic partitioning. This approach simplifies the problem but at the cost of avoiding the intricacies of state sharing among instances.

% Certain frameworks, such as OpenNF~\cite{gember2014opennf}, CHC~\cite{khalid2019correctness}, and others~\cite{woo2018elastic, rajagopalan2013split}, attempt to maintain cross-flow state consistency during execution. However, their solutions are inadequate under dynamic network conditions, including instance failure or traffic reallocation.

% CHC framework~\cite{khalid2019correctness}, despite its intention to fully support COE requirements, suffers from its own limitations. Its coarse-grained approach to managing cross-flow state incurs substantial overhead. Specifically, the framework's decision-making process on caching or flushing state objects, based on upstream traffic partitioner information, results in frequent state object transfers between cache and main memory, inducing high communication overhead. The use of mechanisms such as locks to maintain consistency across multiple instances also introduces additional overhead."

% However, these methods assume \textit{non-shared states} across VNF instances
% The CHC framework~\cite{khalid2019correctness} deserves particular mention as it has made a notable attempt to fully support COE requirements. Nevertheless, its approach to cross-flow state management is coarse-grained, leading to substantial contention overhead. This arises from the mechanism CHC utilizes, which makes decisions on caching or flushing state objects based on state access information from the upstream traffic partitioner, leading to high communication overhead due to the frequent transfer of state objects between the cache and main memory. Additionally, implementing concurrency control mechanisms, such as locks, to handle consistent updates from multiple instances contributes to further contention overhead.

% \subsection{Limitations of Related Works}
% \label{subsec:limitations}
% The realm of Network Function Virtualization (NFV) has seen considerable exploration, with several VNF frameworks proposed~\cite{sherry2015rollback, rajagopalan2013pico, gember2014opennf, khalid2019correctness, woo2018elastic, rajagopalan2013split} to address the challenges of stateful VNF deployment. Despite these efforts, existing frameworks fall short in assuring both efficient VNF state management and \textit{chain output equivalence} (COE) simultaneously.

% Frameworks such as FTMB~\cite{sherry2015rollback}, Pico Replication~\cite{rajagopalan2013pico}, and Split/Merge~\cite{rajagopalan2013split} prioritize state access availability, focusing on failure recovery by discarding state changes or maintaining state availability during traffic reallocation. Nevertheless, these approaches are predicated on the assumption of non-shared states across VNF instances, which does not cater to all real-world scenarios. Contrarily, OpenNF~\cite{gember2014opennf} and S6~\cite{woo2018elastic} recognize the existence of shared states within a single VNF. However, their solutions grapple with the demand for COE requirements, including chain-wide ordering and state consistency during instances' replication and chain-wide failure recovery.

% Addressing shared VNF states while satisfying COE requirements presents significant challenges. Several frameworks~\cite{bremler2016openbox, meng2019micronf, palkar2015e2, rajagopalan2013split, gember2014opennf, khalid2019correctness, woo2018elastic} sidestep these challenges by either disregarding cross-flow states or assuming perfect traffic partitioning, thus avoiding state sharing among instances. Meanwhile, some frameworks make efforts to maintain cross-flow state consistency during execution~\cite{gember2014opennf, khalid2019correctness, woo2018elastic, rajagopalan2013split}, but they falter in dynamic network conditions, such as instance failure or traffic reallocation.

% Among the discussed frameworks, CHC~\cite{khalid2019correctness} is noteworthy for its attempt to fully support COE requirements. However, its coarse-grained cross-flow state management approach comes at the cost of substantial contention overhead. The mechanism utilized by CHC, which involves decisions on caching or flushing state objects based on state access information from the upstream traffic partitioner, engenders significant communication overhead due to the frequent transfer of state objects between the cache and main memory. Furthermore, the implementation of concurrency control mechanisms like locks, necessary for handling updates from multiple instances in a consistent order, contributes to additional contention overhead.

% In Section~\ref{Experiments}, we further investigate the overhead issues linked with CHC's cross-flow state management through detailed experiments.
% \subsection{Limitations of Related Works}
% \label{subsec:limitations}
% \begin{comment}
% \zhonghao{
% Skeleton:
% \begin{itemize}
% \item Overview of existing NFV frameworks: efficiently supporting state management is challenging.
% \item Explain existing state management approaches: OpenNF, Split/Merge, CHC, etc. Even though CHC guarantees COE requirements, it cannot efficiently handle cross-flow states. Conclusion of related works: lack of efficient cross-flow state management.
% \end{itemize}
% }
% \end{comment}

% Stateful VNF deployment has been the focus of various proposed VNF frameworks~\cite{sherry2015rollback, rajagopalan2013pico, gember2014opennf, khalid2019correctness, woo2018elastic, rajagopalan2013split}. Despite their efforts, existing solutions struggle to simultaneously ensure efficient VNF state management and maintain chain-wide correctness as illustrated in Section~\ref{subsec:example}. The majority of these frameworks, including FTMB~\cite{sherry2015rollback}, Pico Replication~\cite{rajagopalan2013pico}, and Split/Merge~\cite{rajagopalan2013split}, prioritize state access availability. These frameworks handle failure recovery by discarding state changes or ensuring state availability during traffic reallocation. However, their design is predicated on the assumption that states are not shared across VNF instances, a situation that is not reflective of all real-world scenarios. OpenNF~\cite{gember2014opennf} and S6~\cite{woo2018elastic} do take shared states into account within a single VNF, yet they struggle to meet chain-wide consistency requirements. These requirements include maintaining chain-wide ordering, as demonstrated in our trojan detector example, and ensuring state consistency during duplicated instance suppression and chain-wide failure recovery.

% However, effectively handling shared VNF states while satisfying COE requirements poses significant challenges for existing NFV frameworks. Some frameworks~\cite{bremler2016openbox, meng2019micronf, palkar2015e2, rajagopalan2013split, gember2014opennf, khalid2019correctness, woo2018elastic} disregard cross-flow VNF states or assume perfect traffic partitioning to avoid state sharing among instances, while others ensure cross-flow state consistency during execution~\cite{gember2014opennf, khalid2019correctness, woo2018elastic, rajagopalan2013split} but struggle to fully support COE requirements under dynamic network conditions like instance failure or traffic reallocation. CHC is the only framework we are aware of that fully supports COE requirements~\cite{khalid2019correctness}. However, we observe that its current cross-flow state management mechanism relies on locking primitives and introduces significant contention overhead during intensive concurrent state access operations, hindering scalability in VNF chains.

% CHC~\cite{khalid2019correctness} is the only framework among those discussed that fully supports all chain-wide correctness requirements. However, its approach involves coarse-grained cross-flow state management, which introduces significant contention overhead. In CHC's method, decisions on caching or flushing cross-flow state objects are based on the state access information from the immediate upstream traffic partitioner. When no updates occur, the state object remains within each instance's cache. If an update request from another instance is detected, the state object is evicted to shared memory, and state update actions are executed. If no further updates are detected, the state object returns to the instance cache. This strategy, despite its apparent effectiveness, incurs considerable overhead in two critical aspects: communication and contention. Frequent updates to shared states necessitate recurrent movement of state objects between the cache and main memory, leading to significant communication overhead. Concurrently, the need to apply updates from multiple instances to state objects evicted to shared memory in a consistent order requires concurrency control mechanisms like locks, which add substantial contention overhead. In Section~\ref{Experiments}, we explore the overhead issues associated with CHC's cross-flow state management through targeted experiments.

==> Sections/Motivating_Example.tex <==
\subsection{Motivating Example}
\label{subsec:example}
\begin{figure}
    \includegraphics[width=\linewidth]{figures/SFC.pdf}
    \caption{An Example NFV Chain.}
    \label{fig:SFC}
\end{figure}
 
Figure~\ref{fig:SFC} shows a representative NFV chain that consists of Network Address Translation (NAT), Load Balancing (LB), and Trojan Detection (TD). Although these functions, deployed sequentially across different Virtual Network Function (VNF) instances, handle distinct packet flows, they rely on shared state objects, which adds complexity to state management in VNFs~\cite{de2014beyond}. Each function operates as follows:

\begin{enumerate}
\item \textbf{Network Address Translation (NAT):} On receiving a new connection, NAT instances select an available port from a shared list and update the per-flow state with the connection's port mapping. Simultaneously, they manage cross-flow states like the available ports and total packet count.
\item \textbf{Load Balancing (LB):} LB instances allocate incoming packets to a suitable server based on its current capacity. They also maintain a connection-to-server mapping and collaborate with other instances to keep track of the active connections and byte count per server.
\item \textbf{Trojan Detection (TD):} TD instances monitor flow timings across different connections on each host to detect Trojan Horse attacks by identifying predefined malicious patterns.
\end{enumerate}

From this operational breakdown of the representative NFV chain, we distill two overarching challenges intrinsic to the management of states in VNFs. The first challenge arising from this example is the need for COE in NFV chains, a concept elaborated in~\cite{khalid2019correctness}. This requirement equates to:
\begin{itemize}
\item \textbf{Availability}:
Every instance in our chain, whether NAT, LB, or TD, must have continuous and up-to-date access to the shared state. This need is crucial even in the face of network fluctuations, such as instance failures or changes in traffic allocation. For instance, if a NAT instance fails, the system should swiftly provide an up-to-date state to the replacement instance to ensure seamless service.
\item \textbf{Consistency}:
Certain instances in our example, like NAT and LB, need to update shared states, including available ports and the active number of connections per server. Synchronizing these concurrent state updates is crucial for maintaining the consistency of shared cross-flow states.
\item \textbf{Ordering}:
In some network functions, it's vital to track the order of incoming traffic. For instance, a TD instance looks for threats based on a specific sequence of network events. Any mix-up in this order, possibly due to network congestion or recovery from failure, can cause incorrect detections. The issue gets more complex with multiple detectors, underscoring the importance of preserving traffic order in managing VNF states.
\item \textbf{Isolation}:
Every module in the NFV chain should be able to recover independently from a failure without causing disruptions in the chain. For instance, if an LB instance fails and recovers, it should not affect the operation of NAT or TD instances.
\end{itemize}

The second challenge resides in the need to maintain execution efficiency while ensuring COE. Particularly in our example, this involves several key components:
\begin{itemize}
    \item \textbf{Concurrent State Access}: Both NAT and LB instances require concurrent reading and updating of shared state objects across multiple instances, such as the available ports list and server capabilities. The absence of adequate synchronization mechanisms could lead to significant contention overhead, affecting efficiency;
    \item \textbf{Dynamic Traffic Conditions}: The NFV Chain must operate under dynamic traffic conditions characterized by frequent instance failures and network bursts. This requires mechanisms capable of discarding associated updates, reverting to a safe state, and efficiently redistributing traffic processing to prevent redundancy. For instance, a sudden surge in traffic could overwhelm the LB instances, necessitating rapid reallocation of traffic to maintain service quality;
    \item \textbf{Cross-flow State Management}: The complexity of managing cross-flow states under such dynamic conditions is a non-trivial task. Given the shared state nature of our example, i.e., available ports, server capabilities, and active connections per server maintaining efficiency while ensuring COE is an intricate challenge.
\end{itemize}
